DAVE: A VLM Vision Encoder for Document Understanding and Web Agents

While Vision-language models (VLMs) have demonstrated remarkable performance across multi-modal tasks, their choice of vision encoders presents a fundamental weakness: their low-level features lack the robust structural and spatial information essential for document understanding and web agents. To bridge this gap, we introduce DAVE, a vision encoder purpose-built for VLMs and tailored for these tasks. Our training pipeline is designed to leverage abundant unlabeled data to bypass the need for costly large-scale annotations for document and web images. We begin with a self-supervised pretraining stage on unlabeled images, followed by a supervised autoregressive pretraining stage, where the model learns tasks like parsing and localization from limited, high-quality data. Within the supervised stage, we adopt two strategies to improve our encoder's alignment with both general visual knowledge and diverse document and web agentic tasks: (i) We introduce a novel model-merging scheme, combining encoders trained with different text decoders to ensure broad compatibility with different web agentic architectures. (ii) We use ensemble training to fuse features from pretrained generalist encoders (e.g., SigLIP2) with our own document and web-specific representations. Extensive experiments on classic document tasks, VQAs, web localization, and agent-based benchmarks validate the effectiveness of our approach, establishing DAVE as a strong vision encoder for document and web applications.

==> appdx_items/vlm_eval/vlm_hparams.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabularx}{0.48\textwidth}{@{} l N @{}}
\toprule
\textbf{Hyperparameter} & \textbf{Value} \\
\midrule
Max Sequence Len     & 20000 \\
Learning Rate  & 3e-5 \\
Epochs         & 2 \\
LR Scheduler   & Step \\
\bottomrule
\end{tabularx}
\caption{Training hyperparameters for Mind2Web.}
\label{tab:alt-hparams}
\end{table}


==> fig/fig1.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/eps_tail_new.pdf}
    \caption{
    \textbf{Inter-parch standard deviation of different data source.}
    Distribution density of the per-patch standard deviation for Imagenet, document, and web images. The y-axis is log-scaled, and the dashed line indicates the numerical floor. We note that the standard deviation of document and web images are heavily concentrated near the floor compared to Imagenet images.
    }
    \label{fig:fig1}
\end{figure}

==> fig/fig3.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{fig/accuracy_ablation_triptych.pdf}
    \caption{
    Analysis of MAE on Document Tasks.
    \textbf{Left: Scaling Resolution.} Performance scale with the resolution of the vision encoder.\textbf{Middle: Scaling Data.} Performance scales with the pretraining data.\textbf{Right: Mask Ratio.} Optimal mask ratio for MAE pretrained on Doc and web images.
    }
    \label{fig:fig4}
\end{figure}

==> sec/experiment_old.tex <==
\section{Evaluation}

\subsection{Datasets}

Here, we provide a description of our training datasets for the different stages.

\minisection{Self-Supervised Learning Data.}
We use 20 million images for our self-supervised training. For document data, we sample 10 million PDF images from DocFM~\citep{team2025granite}, which contains 85 million document pages extracted from Common Crawl, Wikipedia, and ESG (Environmental, Social, and Governance) reports. The PDFs are filtered to include English only. For web screenshot, we sample 10 million from Common-Web~\citep{commonscreens} without any language filtering.

\minisection{Supervised Learning Data.}
For the autoregressive supervised training, we leverage data from diverse sources, including PlotQA \citep{methani2020plotqa}, ChartQA \citep{masry2022chartqa}, fintabnet~\citep{zheng2021global}, Datikz~\citep{belouadi2023automatikz}, Pubtables~\citep{smock2022pubtables}, DocFM \citep{team2025granite}.  Importantly, we use the version from Granite Vision~\citep{team2025granite} where all the problems are reformulated into content extraction. The data for this stage is a mixture of curated benchmarks and a large-scale, self-processed dataset. The curated benchmarks cover tasks such as chart-to-markdown, table-to-caption, and web UI grounding with UGround~\cite{gou2024navigating}. To expand on this, we processed 500K PDF samples from arXiv with an OCR model~\citep{cui2025paddleocr}, formulating them into additional recognition and grounding tasks. Altogether, this training stage comprises approximately 2 million samples.


\minisection{Instruction Tuning Data.}
Following Cambrian-1~\citep{tong2024cambrian}, We use the LLaVA-1.5-mix 665K~\citep{liu2023llava}, DocVQA \citep{mathew2021docvqa}, ChartQA \citep{masry2022chartqa}, and AI2D \citep{Kembhavi2016} as our instruction tuning data. We also integrate Pixmo-Doc \citep{yang2025scaling} into the data mix to improve document understanding. Additionally, we add MultiUI \citep{liu2024harnessingwebpageuistextrich} to improve the web and agentic capability. This combined to a total of 2.5 million training images.

\input{table/tab1}

\subsection{Implementation Details}
\minisection{Self-supervised Stage}
For the SSL stage, we follow the original MAE implementation \citep{he2022masked}, with ViT-L16 \citep{dosovitskiy2020image} as our vision encoder. We train the MAE with a batch size of 4096 for 120K steps. To scale up the resolution to 512 and 768, we finetune the ViT trained with resolution of 384 for an additional 20k steps using the same data.

\minisection{Supervised Training Stage}
We adopt the VLM architecture discussed Section~\ref{sec:prelim}, with an image tilting size of 384. During the ensemble training, we employ frozen SigLIP-2 as the generalist vision encoder, while the encoder from the Self-supervised stage serves as the domain-specialized component. This forms the full \NAME encoder.
We experiment with multiple LLMs of varying scales and architectures, including QWen2.5-0.5B-Instruct \citep{bai2025qwen2}, Phi-4-mini-Instruct \citep{abouelenin2025phi} and Granite-3.1-3B-Instruct \citep{team2025granite}. After a single epoch of full-parameter training, we retain only the \NAME encoder for weight-merging and downstream tasks. During the weight-merging distillation, we train the merge coefficient for 20 epochs. Refer to Appendix~X for implementation detail.


\subsection{Benchmarks}
Here, we provide a description of our evaluation datasets.

\minisection{Classic Document Understanding Tasks}
To directly evaluate the structural and spatial visual representation from the vision encoders, we consider several document parsing tasks that can be performed with only images. We employ DocBank~\citep{li2020docbank} to comprehensively evaluate document recognition on different categories, including tables, charts, and paragraphs. We also use Doclaynet~\citep{pfitzmann2022doclaynet} to test document segmentation. For web tasks, we use RICO-SCA~\citep{li2020mapping} to perform web UI classification.

\minisection{Document and General VQA}
For document understanding and question answering, we evaluate on AI2D \citep{Kembhavi2016}, OCRBench \citep{Liu_2024}, DocVQA \citep{mathew2021docvqa}, InfoVQA \citep{Mathew_2022_WACV}, and ChartQA \citep{masry2022chartqa}. For general vision-language understanding, we report results on MMMU \citep{yue2024mmmu}, RealWorldQA \citep{xai2024realworldqa}, and TextVQA \citep{singh2019textvqa}. 

\minisection{Web UI and Agent Tasks}
For web UI localization, we use Screenspot-V2 \citep{wu2024atlas}, which consists of text instructions, such as click the button, and the corresponding bounding box label. We report the center accuracy, where the center of the label bounding box is within the predicted bounding box. We also evaluate on WebSRC~\citep{chen2021websrc} and VisualWebBench~\citep{liu2024visualwebbench} for web UI question answering. For the agentic benchmark, we evaluate on Mind2Web~\citep{deng2023mind2web}, where the model is given a user goal and a webpage image, and must predict an action like clicking.

\subsection{Evaluation Setting}
\minisection{Baselines}
We compare our vision encoder with both generalist and specialist encoders. For generalist encoders, we utilize DinoV2 \citep{oquab2023dinov2} and Web-SSL MAE \citep{fan2025scaling}, a MAE varient trained on 2 Billion images. We also include SigLIP2 \citep{tschannen2025siglip} and AIMv2 \citep{fini2025multimodal}, which are SOTA encoder trained with both contrastive and reconstruction. For specialist vision encoders, we compare against DiT~\citep{li2022dit}, Pix2Struct \citep{lee2023pix2struct}, and Dolphin \citep{feng2025dolphin}. Since both Pix2struct and Dolphin are encoder-decoder models, we use their encoder for comparison.

\input{table/tab2}

\minisection{Task-specific Finetune}
For each classic document image parsing task, we finetune the vision encoder and the suitable prediction heads. In DocBank, we use attention pooling to pool to visual feature followed by an MLP head predict the bounding box. Each category is trained separately. In Doclaynet, we train an MLP head to predict the semantic segmentation based on the feature patches. For RICO-SCA, we use attention pooling followed by an MLP to predict the class.
\input{table/tab3}

\minisection{Vision-Language Model as Evaluator}
To evaluate our vision encoders on more complicated and realistic tasks, such as VQA and instruction-based localization, we use VLMs as evaluator. Specifically, we follow the standard LLaVA architecture as discussed in Section~\ref{sec:prelim}. We use a a tilting size of 336 for AIMv2 and 384 for all other vision encoders. For vision encoders that produce different number of visual tokens than the tilting resolution, we use bilinear interpolation as in LLaVA-Onevision~\citep{li2024llava} to interpolate the visual tokens. Note that we omit the projector alignment phase to improve training efficiency, as prior work has shown that this stage yields only limited gains~\cite{tong2024cambrian, karamcheti2024prismatic}. We use Llama-3.2-3B-Instruct~\citep{dubey2024llama} and Qwen2.5-7B-Instruc~\citep{bai2025qwen2} as the LLM backbone. We train for one epoch with the vision encoder frozen. For Mind2web, we finetune the VLMs on the training set before performing offline evaluation on test set. More detail can be found in Appendix~X.
